Emotional Speech-Driven Animation with Content-Emotion Disentanglement

To be widely adopted, 3D facial avatars must be animated easily, realistically, and directly from speech signals. While the best recent methods generate 3D animations that are synchronized with the input audio, they largely ignore the impact of emotions on facial expressions. Realistic facial animation requires lip-sync together with the natural expression of emotion. To that end, we propose EMOTE (Expressive Model Optimized for Talking with Emotion), which generates 3D talking-head avatars that maintain lip-sync from speech while enabling explicit control over the expression of emotion. To achieve this, we supervise EMOTE with decoupled losses for speech (i.e., lip-sync) and emotion. These losses are based on two key observations: (1) deformations of the face due to speech are spatially localized around the mouth and have high temporal frequency, whereas (2) facial expressions may deform the whole face and occur over longer intervals. Thus, we train EMOTE with a per-frame lip-reading loss to preserve the speech-dependent content, while supervising emotion at the sequence level. Furthermore, we employ a content-emotion exchange mechanism in order to supervise different emotions on the same audio, while maintaining the lip motion synchronized with the speech. To employ deep perceptual losses without getting undesirable artifacts, we devise a motion prior in the form of a temporal VAE. Due to the absence of high-quality aligned emotional 3D face datasets with speech, EMOTE is trained with 3D pseudo-ground-truth extracted from an emotional video dataset (i.e., MEAD). Extensive qualitative and perceptual evaluations demonstrate that EMOTE produces speech-driven facial animations with better lip-sync than state-of-the-art methods trained on the same data, while offering additional, high-quality emotional control.

==> bk_02_related.tex <==

\section{Related Work}
\label{sec:related}
\yandong{I guess this part need to be reorganized. We could keep the motion prior, semantic control, supervision, 2D talking head parts. We might also need to add discussion of lip-reading and emotion. Architecture is TBD.}

\subsection{3D Talking Head Generation}
Speech-driven 3D facial animation can be separated into two lines of research. 
Procedural  \todo{machine gun of citations} and data-driven. 
Here we only focus only on the deep learning based line of work. 
While the field has a long history \cite{cao2005expressive} \todo{add old school data driven methods}, the most relevant recent works leverage deep learning \cite{pham2017end, pham2017speech, karras2017audio, cudeiro2019capture, richard2021meshtalk, fan2022faceformer, xing2023codetalker}. 
Next we discuss the individual features of the most relevant methods.

\paragraph{Input representation:} \todo{maybe minor and sufficient to clarify this in the method section?}
Some methods train their own specific audio encoders, usually different variations of temporal convolutional networks ~\cite{pham2017end, pham2017speech, karras2017audio, richard2021meshtalk}. %Karras et al.~\cite{karras2017audio} train a temporal convolutional net on the raw waveform. Richard et al.~\cite{}.
Other methods instead leverage a pretrained speech representation net. 
Cudeiro et al.~\cite{cudeiro2019capture} use a pretrained and frozen automatic speech recognition (ASR) network that outputs per-character probabilities (DeepSpeech  \cite{hannun2014deep}). 
Fan et al.~\cite{fan2022faceformer} and our leverage self-supervised transformer-based Wav2Vec 2.0 \cite{baevski2020wav2vec} and further finetune it. 
We follow the same approach.

\paragraph{Output representation:} \todo{maybe minor and sufficient to clarify this in the method section?}
Most of the prior methods predict 3D vertices \cite{karras2017audio} or vertex displacements \cite{cudeiro2019capture, richard2021meshtalk, fan2022faceformer} in full space. 
As such, they do not leverage facial shape models explicitly. 
Only \cite{pham2017end, pham2017speech} leverage a 3DMM. However, their 3DMM is low quality and does not factor expression and identity. 
Our work is, to the best of our knowledge, the first to leverage a high quality statistical shape model FLAME \cite{FLAME:SiggraphAsia2017} as its output space. 
This comes with many advantages, ranging from compressed representation to the factored and editable representations shape, expression and jaw pose. 

\paragraph{Architecture:} \todo{maybe minor and sufficient to clarify this in the method section?}
All methods follow an encoder-decoder type of architecture. Different methods leverage different macro-architectural blocks such as temporal convolutions \cite{karras2017audio, cudeiro2019capture}, LSTMs \cite{richard2021meshtalk} and most recently transformers \cite{fan2022faceformer}. 
We also use a transformer-based approach but instead for an autoregressive transformer decoder used in Faceformer \cite{fan2022faceformer}, we opt for a BERT-like feedforward transformer design.

\paragraph{Motion prior:} 
Most methods do not learn or apply any type of motion prior and let the space of valid motions be learned by the architecture itself from the training data \cite{pham2017end, pham2017speech, karras2017audio, cudeiro2019capture, fan2022faceformer}.
MeshTalk \cite{richard2021meshtalk} on the other hand, adopts a two-stage approach. In the first stage a motion prior with a categorical latent space is trained. 
This pretrained prior is the utilized in the second stage for the autoregressive generation of the results. 
Our method also makes use of a motion prior but out motion prior is a continuous VAE and unlike MeshTalk that does not enforce any temporal compression, a single latent vector of our motion prior models motion of several frames.
CodeTalker \cite{xing2023codetalker} adopts a similar approach to FaceFormer \cite{fan2022faceformer} and augments it with a separately trained VQ-VAE for motion prior.

\paragraph{Generalization:} \todo{maybe redundant with the following paragraphs?}
Karras et al.~\cite{karras2017audio} rely on high fidelity scans of a single individual to train a person-specific model and as such can easily learn the subject's speaking style and idiosyncracies.
~\cite{cudeiro2019capture, fan2022faceformer} use a multi-person dataset and condition the generation with an ID of the speaker, resulting in generation of speaking style of the given training subject. 
% The style in question is learned jointly in training.
Richard et al.~\cite{richard2021meshtalk} take a probabilistic autoregressive approach simlar to R-CNN \cite{pixelcnn}. 
This is enabled by the large dataset with over 250 subjects that encapsulates many different speaking styles.

\paragraph{Deterministic vs Probabilistic:}
Nearly all the works adopt a fully deterministic \cite{pham2017end, pham2017speech, karras2017audio, cudeiro2019capture, richard2021meshtalk, fan2022faceformer} approach.
As such, these methods fail to model the fact that the mapping from speech audio to facial animation is non-deterministic which results in reduced expressivity.
MeshTalk \cite{richard2021meshtalk} in turn learns a categorical latent space that is then autoregressively sampled and therefore capable of generating multiple plausible animations per speech track.

\paragraph{Semantic control:}
Almost none of the existing methods provide the user with a semantically meaningful way of control over the result. 
VOCA \cite{cudeiro2019capture} and FaceFormer \cite{fan2022faceformer} allow for speaking style control by interpolating style vectors of training individuals, which is not very user-friendly. 
While the probabilistic autoregression of MeshTalk \cite{richard2021meshtalk} allows the generation of a variety of results for the same input, there is no mechanism that allows for any control of emotion or style.
Karras et al.~\cite{karras2017audio} do learn a type of emotional latent space by jointly learning a feature vector for each training sample in an unsupervised way. 
Changing this feature vector then allows for test time editing. 
While yielding promising results, the learnt space does not inherently contain a semantic meaning and must be manually assigned after careful inspection after training.
Furthermore, since there is no disentanglement mechanism, the model lacks the guarantee that mixing different emotion vectors with different audio inputs results in the desired result (correct lipsync and desired emotion) since there is no mechanism that supervises it.
In contrast to that, our method is - to the best of our knowledge - the first to factorize the effect of emotion and speech on the resulting 3D animation via a novel emotion-content disentanglement mechanism, allowing for automatic semantically meaningful emotion editing at test time.

\paragraph{Supervision:}
All of the recent methods are fully supervised \cite{karras2017audio, cudeiro2019capture, richard2021meshtalk, fan2022faceformer, bala2022imitator} in that they require a dataset of 3D scans paired with synchronized speech audio in order to be trained. 
Most notably, the methods rely on mean squared error loss between the predicted and GT vertices (or vertex offsets) enforced for each frame.
Karras et al.~\cite{karras2017audio} add an additional regularization term to ensure the smoothness of their emotional database.
Richard et al.~\cite{richard2021meshtalk} introduce a cross-modal loss to enforce reconstruction of audio-correlated and uncorrelated information separately in order to learn their categorical motion prior and an explicit eye close loss to enforce eyeblinks.
Furthermore, 
Thambiraja et al.~\cite{bala2022imitator} introduce a mouth closure loss that is active only when bilabials are spoken which helps achieve correct mouth closure.
In our work, we apart from a supervised MSE loss, we additionally utilize perceptual lip and emotion consistency losses.


\todo{incorporate Bala's work \cite{bala2022imitator}}

\todo{Incorporate Learning to listen}


% VOCA \cite{cudeiro2019capture} uses a pretrained and frozen automatic speech recognition (ASR) network that outputs per-character probabilities (DeepSpeech \cite{hannun2014deep}) and these are then mapped to per vertex displacements using temporal convolutions followed by an MLP. 
% Like VOCA, Faceformer by Fan et al.~\cite{fan2022faceformer} uses a pretrained automatic speech recognition net (wav2vec 2.0 \cite{baevski2020wav2vec}) which is then finetuned along with an autoregressive transformer decoder and modified biased attention mechanism. 
% FaceFormer is the current SOTA on VOCASET in terms of per-vertex error.
% % Faceformer is the first method that utilizes transformers.  
% FaceFormer is perhaps the most similar approach to \model. 
% Like FaceFormer, \model uses a pretrained wav2vec 2.0 for speech feature extraction.
% Unlike FaceFormer, \model does not make use of the auto-regressive transformer decoder which we found quite inefficient due to the autoregressive loop. 
% A BERT-like decoder is used instead, which allows \model to predict all animation frames in one pass.

% While the aforementioned methods can produce good mouth articulation, they fail to animate the rest of the face. 
% This results in uncanny effects of such as a fixed neutral expression or missing eye blinks. 
% MeshTalk \cite{richard2021meshtalk} attempts to alleviate this problem by learning a categorical latent space that disentangles speech correlated and uncorrelated information. 
% In addition to this, since MeshTalk utilizes a variational approach, which makes the generation of multiple plausible motions per speech-track possible. \todo{Verify that this is correct}

% \todo{cite \cite{pham2017end, pham2017speech}}

% \todo{Keep only if we make it variational} None of the existing methods, however, put any emphasis on semantic control of the animation. \cite{cudeiro2019capture, fan2022faceformer} are fully deterministic and the only control from speaking style is achieved through a one-hot encoding which corresponds to the index of a subject from the training set. 

% To the best of our knowledge, no data-driven method has ever made use of an existing 3DMM but instead learned the deformation space only from the dataset used for training. 
% In contrast to that, \model makes use of the FLAME model \cite{FLAME:SiggraphAsia2017}.


% Also, MeshTalk \cite{richard2021meshtalk} does not provide any semantic way to control the generation process, beyond autoregressively sampling from the categorical space. 
% The approach of Karas et al.~\cite{karras2017audio} allows for a certain degree of control as their training also includes an automatic latent space learning for the training examples. 
% This latent can then be changed at test time. 
% However, this control is not intuitive and can only be applied to a single subject.
% Hence, none of these models have any means of giving the user some form of semantic control such as the ability to change the emotion. 



% A recent work by Ng et al.~\cite{ng2022learning2listen} uses the speech input in a less conventional way. Instead of the speaker, the speech audio (along with the speaker motion) is used to animate the listener character.

\subsection{2D talking head generation}

The field of 2D talking head generation, i.e. how to generate a video using speech received a tremendous amount attention in recent years thanks to the abundance of face video data. 
% The methods usually relies on conditioning an image generation network in order to control the resulting video. 
% Some models are person specific \todo{machine gun of citations} and some general to multiple subjects \todo{machine gun of citations}.
These methods could be separated into two mines lines of work - purely 2d-based methods \cite{AverbuchElor, tripathy2019icface, Zakharov2019, kim2019neural, chen2019hierarchical, choi2020starganv2, Ding2017ExprGANFE, lindt19, dApolito_2021_CVPR, ji2021evp, cheng2022VideoReTalking, Tripathy_2021_facegan} and those with and underlying 3D model driving the result video \cite{thies2015realtime, thies2016face, kim2018deep, head2head2020, Ghosh2020, thies2020nvp, paraperas2022ned}. % \todo{machine gun of citations}.

An in-depth review of all these is beyond the scope of this paper. 
Instead we briefly review the most relevant to our method - 3D aware methods and emotion aware methods. 

\paragraph{3D aware:}
Neural emotional director (NED) \cite{paraperas2022ned} utilizes 3D faces under the hood. DECA \cite{Feng2021_DECA} reconstructions are manipulated with a 3D-based emotion manipulator that modifies the expression parameters of the shape before rendering it with a differentiable renderer and subsequently postprocessing the image with a translation net.

\todo{Neural voice puppetry \cite{thies2020nvp}, wav2lip \cite{praywal2020wav2lip}, adnerf \cite{guo2021adnerf}, }


\paragraph{Emotion aware:}
Emotional video portrait \cite{ji2021evp}.

% The goal of NED \cite{paraperas2022ned} is similar to our work, to control the emotion while keeping the articulation plausible for a given audio. 
NED \cite{paraperas2022ned} is similar to our work in that aims to modify the emotion of a speaker in an in-the-wild video whilst preserving the speech.
It does so by changing the expression parameters of DECA \cite{Feng2021_DECA} reconstructions using a StarGanV2 \cite{choi2020starganv2} inspired translation network. 
Thanks to the StarGAN-like formulation, it can translate a reconstruction sequence to match the style of one of the basic emotions.
The idea is that the style vector explains the emotion while the content (articulation) preservation is handled by the cycle-consistency loss. 
Since NED is inherently limited by the lack emotional expressivenes of DECA, the resulting shapes are most likely also limited in their emotion and lip sync.
The authors do not showcase the edited shapes separately, only the resulting neural renderings, making it hard to judge the quality of the edited geometry separately.

\todo{paper GANmut}

\todo{ICface} 

\todo{DSM}


% \todo{begin: written by Kiran}
% Chen et al.~\cite{chen2019hierarchical} and Yu et al.~\cite{8995571} proposes a hierarchical approach to learn landmarks from multimedia inputs and generate video frames from landmarks. Eskimez et al.~\cite{seeskimezemotface} uses an emotion encoder for one-hot vector as emotion label and generates talking face conditioned on speech and a single face image using a GAN architecture. In 2D talking face generation, Song et al.~\cite{linsen2020ebt} method uses 3D parametric face reconstruction method to orthogonal geometry and pose information and uses speech encoding network for expression parameters extraction. Using a conditional input, they generate a 2D talking face by using a dynamic-programming based rendering network.

% Triantafyllos et al.~\cite{Kefalas2020SpeechDrivenFA} introduces a concept of modeling first-order and second-order polynomial interaction matrices for audio and identity to generate 2D talking face. The work proposed by Ji et al.~\cite{10.1145/3528233.3530745} included emotion extraction from arbitrary source video and transferring the emotional face displacements to source image and audio to generate talking faces by predicting unsupervised motion representations. Liu et al.~\cite{liu2022semantic} explores Neural Radiance Fields (NeRF) for audio driven video generation by combining semantic aware dynamic ray sampling with torse deformation implicit function to capture association between lip and torso movements. Yin et al.~\cite{2203.04036} demonstrates extracting feature maps by the flow motion fields. In this work, the motion fields are calibrated using pre-trained StyleGAN to generate talking face with either a driving video or an audio. 
% q
% By disentangling audio representation, Park et al.~\cite{Park_Kim_Hong_Choi_Ro_2022} proposes audio-lip movement memory mapping along-with visual-visual synchronization between ground truth and predicted face to generate 2D talking faces. Ye et al.~\cite{DBLP:journals/corr/abs-2204-06180} allows to generate talking face video and continuously control expressions by dynamically generating 3DMM-based neural textures. Zhang et al.~\cite{zhang2021facial} is a GAN-based approach to synthesize 2D talking faces with audio-synchronized lip motion, head motion, and eye blinks. Zhou et al.~\cite{zhou2021pose} devises a low-dimensional pose code for speech content, head pose and identities. Further these features are assembled to generate 2D talking faces using adversarial generative training.  Li et al.~\cite{Li_Wang_Zhang_Ding_Zheng_Yu_Fan_2021} models facial expressions and head animations from textual input in two stages. In the first stage, it maps text into mouth, upper face, and head pose animation parameters, whereas in the second stage these parameters are used to rig to the input speaker's facial landmarks. The model presented in Wang et al.~\cite{wang2021audio2head} uses a recurrent network based head motion predictor and motion field generator to produce keypoints that govern the spatial and temporal consistency of generated videos.  

% Zhou et al.~\cite{Yang:2020:MakeItTalk} generates speaker-aware talking head 2D animation by first disentangling speech features in speaker identity and content embedding. The predicted landmarks using these embedding along-with the source image facial landmarks are together used to drive the 2D talking head motion dynamics.  Thies et al.~\cite{thies2020nvp} employs a content aware audio feature filtering on per-frame audio features. Trained on audio features and the 3D tracking performed on corresponding "in-the-wild" videos, the network predicts the generic blendshape basis of the statistical face model, which is rendered to a 2D talking face video output.

% \todo{end: written by Kiran}


% \subsection{Probabilistic talking head generation}

% \todo{proofread and add more if necessary or remove altogether}
% Jonell et al.~\cite{10.1145/3383652.3423911} is a normalizing flow based interlocutor aware facial gesture generation model conditioned on avatar's speech features and interlocutor's facial gesture and speech features. The architecture proposed in Liang et al.~\cite{9878472} granularly encodes pose, expression, content, identities, and audio separately and assembles to generates talking face videos using generator network inspired from Burkov et al.~\cite{Burkov_2020_CVPR} that employs adaptive instance normalization Huang et al.~\cite{huang2017adain} for fast approximation of style transfer. Chen et al.~\cite{https://doi.org/10.48550/arxiv.2110.09951} is a generative talking head method that fuses audio and speech related action units by a non-causal temporal convolution self-attention network. Wu et al.~\cite{wu2021imitating} introduces generation of stylized talking 3D heads and 2D videos by devising a latent style fusion model to imitate styles from the style code.  

% \subsection{Audio representations for talking head}

% \todo{proofread and add more if necessary}
% Mittal and Wang~\cite{DBLP:conf/wacv/MittalW20} introduces disentangling audio representations into content, emotions, background noise and others using LSTM-based VAE architecture to demonstrate robustness to emotional variations in talking head generation. Ji et al.~\cite{ji2021audio-driven} work allows to disentangle content-agnostic emotion feature to predict face landmarks and 2D talking videos. 

\subsection{Datasets} 
\paragraph{3D Datasets:}
The ideal dataset for our task would 
%Datasets suitable for 3D talking head generation must 
contain ground-truth (GT) 3D face scans synchronized with audio. 
Such data is limited due to the expense and complexity involved in capture it.
%There are not many datasets of this kind due to the lengthy and expensive process one most go through in order to acquire them.  
BIWI \cite{eth_biwi_00760}, VOCASET~\cite{cudeiro2019capture}, S3DFM~\cite{10.1016/j.sigpro.2019.02.025}, and Multiface~\cite{richard2021meshtalk} are publicly available datasets for the audio-driven 3D talking head task. 
These datasets are limited in size, richness of emotion, speaking styles, and shapes of the subjects.
%Hence, we turn our attention to 2D datasets.

% Old commented content below:
% BIWI \cite{eth_biwi_00760} introduced by Fanelli et al.~is one such dataset. 
% BIWI contains 3D meshes and audio correspondences of 14 speakers and emotion labels for sequences. 
% However, the quality of the 3D shapes is very low.
% Cudeiro et al.~\cite{cudeiro2019capture} released VOCASET which is a high quality dataset of scanned face meshes with synchronized audio of 12 speakers amounting to roughly 29min of footage. 
% However, the dataset only contains normal speech. 
% Richard et al.~\cite{richard2021meshtalk} used the largest scanned dataset for their work MeshTalk. The dataset consists of 250 subjects reading 50 phonetically balanced sentences, amounting to about 13 hours of data. 
% Unfortunately, this dataset has not been publicly released.
% In summary, the publicly available datasets for the audio-driven 3D talking head task are insufficient in size, richness of emotion, speaking styles and shapes of the subjects.
% Hence, we turn our attention to 2D datasets.

\paragraph{2D Datasets:}
% \todo{Compress this section}
In contrast to the limited richness of 3D datasets, 2D video is plentiful.
Off-the-shelf 3D face reconstruction methods can be applied to the video frames, providing pseudo-GT data.
%An alternative to capturing 3D datasets is using video face datasets coupled with 
%off-the-shelf reconstruction methods for faces in-the-wild and use the reconstructions as pseudo-GT. 
This, however, comes with many drawbacks. 
While the field of image-based 3D face reconstruction has made tremendous progress \cite{Deng2019,Genova2018,Tewari2017,Tewari2018,Tewari2019_FML, Sanyal2019_RingNet,Feng2021_DECA,Shang2020_MGCNET,yang2020facescape, EMOCA:CVPR:2021, filntisis2022visual, MICA:ECCV2022}, even the state-of-the-art (SOTA) methods are often not robust to many in-the-wild conditions like occlusion, have inaccurate shape or expression reconstruction, or are not temporally stable . 
%However, 2D image video datasets are much more common, as they can be captured more easily or gathered on the internet. 
Despite these limitations, the large amount of data available from video outweighs the downsides.
%Since there is no 3D dataset that provides us with sufficient amount of data for our goal, we opt to utilize 2D video datasets instead.
Consequently, we generate pseudo-GT data from video by integrating three recent SOTA methods \cite{EMOCA:CVPR:2021, MICA:ECCV2022, filntisis2022visual}.

There are many available video-speech datasets \cite{nagrani2017voxceleb,Chung2018_VoxCeleb2,roessler2018faceforensics,zhu2022celebv,afouras2018deep,afouras2018lrs3,wang2021facevid2vid,kaisiyuan2020mead}.
VoxCeleb1 \cite{nagrani2017voxceleb},  VoxCeleb2 \cite{Chung2018_VoxCeleb2}, Faceforensics++ \cite{roessler2018faceforensics}, Celeb-VHQ \cite{zhu2022celebv}, LRS2 \cite{afouras2018deep}, LRS3 \cite{afouras2018lrs3}, TalkingHead-1KH \cite{wang2021facevid2vid}, and MEAD \cite{kaisiyuan2020mead} are publicly available video datasets. 
There are also video datasets focused Speech Emotion Recognition (SER) \cite{livingstone2018ryerson,cao14_crema,poria2018meld,cmumosi,cmumosei}.
Similarly, RAVDESS \cite{livingstone2018ryerson}, CREMA-D \cite{cao14_crema} , MELD \cite{poria2018meld}, CMU-MOSI \cite{cmumosi} and CMU-MOSEI \cite{cmumosei} are video datasets previously used in the Speech Emotion Recignition (SER) field. 
Of the above, the MEAD dataset  \cite{kaisiyuan2020mead} is of sufficient size, captured in the lab and therefore easier for off-the-shelf face reconstruction and, most of all, exhibits high emotional variety. 

% \begin{table}[t]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \input{tables/datasets_table}}
% \caption{{\bf Datasets}}
% \label{table:data}
% \end{table}

% We outline all dataset information in Table \ref{table:data}. In summary, the challenges of using video datasets are many. 
% While there is seemingly many datasets available, each of them come with a particular set of challenges (such low video quality, too difficult for face reconstruction, not enough variety etc.). 
% Taking all of the above into account, we opt for using MEAD in our experiments.

% Old commented content below:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Face video datasets are much more abundant. 
% VoxCeleb1 \cite{nagrani2017voxceleb} and VoxCeleb2 \cite{Chung2018_VoxCeleb2} are video datasets of talking celebrities designed for the speaker recognition task which together amount to about 1200 speakers in over 21 thousand videos of more than 145 thousand utterances each. 
% While this size is more than abundant, many of these videos are quite low resulotion or suffer from video compression artifacts which makes them suboptimal for pseudo-GT extraction.
% Faceforensics++ \cite{roessler2018faceforensics} and CelebV are not large enough in scale and richness and present similar image quality issues.

% % \todo{Faceforensics++}

% % \todo{CelebV}

% Video datasets designed for the lip reading task such as 
% % LRW \cite{chung2017lip} (, 
% LRS2 \cite{afouras2018deep} and LRS3 \cite{afouras2018lrs3} (over 150 utterances each) are also very relevant. 
% However, the conent of these videos is seldom emotional, as the content comes from BBC television and TED talks respectively. 
% Furthermore, due to the lip reading task, the videos are processes such that they are centered and cropped around the mouth and often miss a considerable amount of the forehead region. 
% Also, similarly to the with VoxCeleb datasets, the video quality is often very limited. 

% Perhaps surprisingly, there are datasets used in the speech emotion recognition field (SER), that also come with video such as
% RAVDESS \cite{livingstone2018ryerson}, CREMA-D \cite{cao14_crema} , MELD \cite{poria2018meld}, CMU-MOSI \cite{cmumosi} and CMU-MOSEI \cite{cmumosei}.
% Most of these, however, are either too small \cite{cmumosi, cao14_crema} or not of sufficient variety in terms of number of utterances \cite{livingstone2018ryerson}, speakers \cite{livingstone2018ryerson, poria2018meld}, resolution \cite{cao14_crema, poria2018meld}. % or their raw videos are not publicly available \cite{cmumosei}.

% \todo{Datasets from Affective computing} AffWild2, AFEW, AFEV-VA,  SEWA, SEMAINE, VAM, ... are they even worth mentioning?
% % http://multicomp.cs.cmu.edu/resources/cmu-mosei-dataset/

% Celeb-VHQ \cite{zhu2022celebv} is a new recent video dataset of faces in-the-wild with over 35 thousand videos of more than 15 thousand people. 
% While the video quality of this dataset is quite high compared to the other datasets, many of the videos are too challenging for the contemporary face reconstruction methods due to challenging environments, occlusions etc. 
% Furthermore, the audio in the videos does not contain only the speaker in question but also other sources of noise (background noise, other speakers, music etc.). 

% TalkingHead-1KH \cite{wang2021facevid2vid} contains over 500 thousand clips, many of them of high resolution and is specifically designed for the 2D talking head generation task.
% Still, not many of the videos contain highly emotional content. \todo{Verify this}.


% MEAD \cite{kaisiyuan2020mead} is a dataset of 48 identities, each about 30 videos each all 8 basic emotions in three intensities captured in a lab. 
% Totalling over 11500 of short videos with over 30 hours of footage. 
% The dataset is of sufficient size, captured in the lab and is therefore a lesser challenge for off-the-shelf face reconstruction and, most of all, exhibits high emotional variety. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Style-controlled full-body animation}

% \todo{proofread and change placing}
% Several works considers speech-driven full-body gesticulation work with latent space modification for style changes. Ghorbani et al.~\cite{https://doi.org/10.48550/arxiv.2209.07556} proposes a variational framework that learns and can modify a style embedding to generate animation with zero-shot style control by example. Habibie et al.~\cite{gesturematching22} generates controllable 3D gestures using database matching for plausible prediction and c-GAN model for audio-driven refined gesture generation.  In this work, Taylor et al.~\cite{10.1145/3485441.3485647} FLOW-VAE model is used to speech-driven gesture animation. Our work is inspired by style controllable gesture synthesis, however our focus as opposed to is towards emotion-controllable speech-driven facial animation. 


==> tables/generation_table.tex <==
\begin{tabular}{l|c|cccc}
\toprule
    Model               &   ER Accuracy $\uparrow$       &  WER $\downarrow$ &  CER $\downarrow$ &  VWER $\downarrow$ &  VCER $\downarrow$  \\
\midrule
    FaceFormer (orig)   &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FaceFormer (ours)   &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FaceFormer-Emo      &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FlameFormer         &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FlameFormer-Emo     &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FlameBERT           &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    \model\!-raw         &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    \model             &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
\bottomrule
\end{tabular}


==> tables/lrs3_generated_emo.tex <==
\begin{tabular}{lllll}
\toprule
           model & emotion accuracy & emotion F1 \\
\midrule
           EMOTE &            0.426 &      0.292 & \\
   EMOTE w/o dis &            0.330 &      0.222 & \\
   EMOTE w/o emo &            0.375 &      0.226 &   \\
   EMOTE w/o lip &            0.256 &      0.112 &   \\
 EMOTE w/o FLINT &            0.432 &      0.298 &   \\
    EMOTE w/o pl &            0.304 &      0.195 &  \\
EMOTE /w st. emo &            0.378 &      0.228 &   \\
% \todo{Faceformer-EMO}
\bottomrule
\end{tabular}


==> tables/reconstruction_table.tex <==
\begin{tabular}{l|c|c|cccc}
\toprule
    Model               &   Vertex MSE $\downarrow$ &   ER Accuracy $\uparrow$         &  WER $\downarrow$ &  CER $\downarrow$ &  VWER $\downarrow$ &  VCER $\downarrow$  \\
\midrule
    FaceFormer (orig)   &   todo                    &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FaceFormer (ours)   &   todo                    &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FaceFormer-Emo      &   todo                    &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FlameFormer         &   todo                    &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FlameFormer-Emo     &   todo                    &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    FlameBERT           &   todo                    &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    \model\!-raw         &   todo                    &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
    \model             &   todo                    &   todo                         &  TODO             &  TODO             &  TODO              &   TODO              \\
\bottomrule
\end{tabular}

